Do LLMs Reproduce the Age Gap in Loneliness? Evaluating Survey Simulation against European Survey Data

Large language models (LLMs) are often used to simulate survey respondents, but matching survey averages does not establish accurate demographic differences. We test whether LLM outputs reproduce within-country age gaps in loneliness using the 2022 EU Loneliness Survey, comparing adults aged 18-34 and 65 or older in France, Italy, Poland, and Sweden. We evaluate simulation with and without age information and direct distribution estimation against a probability-based sample, with a non-probability sensitivity reference. Both human samples show higher mean loneliness among younger adults. Under age-specified simulation with standard response-option order, Mistral Small 4 and GPT-5.6 Terra reverse this ordering under all three prompt framings in three and two countries, respectively, mainly by overestimating older-adult means. DeepSeek V4 Flash preserves the ordering everywhere but underestimates both group means, with errors largely cancelling in France and Italy. Against the probability-based reference, direct estimation has lower absolute age-gap error than simulation for Mistral and Terra in every country. For DeepSeek, simulation has lower gap error but direct estimation has lower group-mean error; these comparisons depend on low-validity older-adult simulation cells. Evaluating LLM outputs as proxies for age groups within countries therefore requires checking both group means and their contrast against human survey data.

==> tables/human_reference.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{7pt}
\begin{tabular}{@{}lcccccc@{}}
\toprule
 & \multicolumn{2}{c}{$n$ ($n_{\mathrm{eff}}$)} & \multicolumn{2}{c}{Mean} & \multicolumn{2}{c}{Gap} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(l){6-7}
 & 18--34 & 65+ & 18--34 & 65+ & Est. & 95\% CI \\
\midrule
\multicolumn{7}{@{}l}{\textit{EU4 (probability-based)}} \\
France & 196 (138) & 271 (168) & 5.05 & 4.06 & $-$1.00 & [$-$1.36, $-$0.62] \\
Italy & 176 (102) & 263 (163) & 5.09 & 4.19 & $-$0.89 & [$-$1.31, $-$0.49] \\
Poland & 219 (93) & 98 (70) & 5.38 & 4.27 & $-$1.10 & [$-$1.63, $-$0.57] \\
Sweden & 203 (196) & 294 (290) & 5.25 & 3.95 & $-$1.30 & [$-$1.59, $-$1.02] \\
\addlinespace
\multicolumn{7}{@{}l}{\textit{EU27 (non-probability online; matched countries)}} \\
France & 232 (148) & 202 (133) & 4.91 & 4.39 & $-$0.52 & [$-$0.92, $-$0.12] \\
Italy & 198 (122) & 223 (164) & 5.74 & 4.39 & $-$1.35 & [$-$1.79, $-$0.90] \\
Poland & 262 (193) & 90 (64) & 5.36 & 4.51 & $-$0.84 & [$-$1.35, $-$0.31] \\
Sweden & 269 (224) & 206 (163) & 5.74 & 3.95 & $-$1.79 & [$-$2.11, $-$1.46] \\
\bottomrule
\end{tabular}
\caption{Human reference from the EU Loneliness Survey 2022. $n$: respondents after exclusions; $n_{\mathrm{eff}}$: Kish effective sample size. Means are weighted UCLA-3 scores (range 3--9). Gap: 65+ minus 18--34; negative values mean younger adults report more loneliness. Older group: ages 65--100. Intervals: 95\% fixed-weight respondent percentile bootstrap, 10{,}000 resamples within each sample--country--age group.}
\label{tab:human-reference}
\end{table*}

